IPCV: Information-Preserving Compression for MLLM Visual Encoders

Multimodal Large Language Models (MLLMs) deliver strong vision-language performance but at high computational cost, driven by numerous visual tokens processed by the Vision Transformer (ViT) encoder. Existing token pruning strategies are inadequate: LLM-stage token pruning overlooks the ViT's overhead, while conventional ViT token pruning, without language guidance, risks discarding textually critical visual cues and introduces feature distortions amplified by the ViT's bidirectional attention. To meet these challenges, we propose IPCV, a training-free, information-preserving compression framework for MLLM visual encoders. IPCV enables aggressive token pruning inside the ViT via Neighbor-Guided Reconstruction (NGR) that temporarily reconstructs pruned tokens to participate in attention with minimal overhead, then fully restores them before passing to the LLM. Besides, we introduce Attention Stabilization (AS) to further alleviate the negative influence from token pruning by approximating the K/V of pruned tokens. It can be directly applied to previous LLM-side token pruning methods to enhance their performance. Extensive experiments show that IPCV substantially reduces end-to-end computation and outperforms state-of-the-art training-free token compression methods across diverse image and video benchmarks. Our code is available at https://github.com/Perkzi/IPCV.

==> Contents/abstract_v2.tex <==
% To overcome these challenges, we introduce IPCV, a \textbf{training-free, information-preserving compression} framework for MLLM visual encoders. IPCV facilitates aggressive token pruning within the ViT by employing a novel \textbf{Neighbor-Guided Reconstruction (NGR)} mechanism. NGR allows pruned tokens to be temporarily reconstructed to participate in attention with minimal overhead, and then fully restores them before they enter the LLM. This semantic recovery step ensures that a complete and high-fidelity set of visual features is available for downstream multimodal reasoning. Paired with a lightweight LLM-stage pruner, IPCV's dual-stage design maximizes computational savings while preserving semantic integrity. Extensive experiments demonstrate that IPCV substantially reduces end-to-end computation and outperforms state-of-the-art training-free token compression methods on a wide range of image and video benchmarks.
%
Multimodal Large Language Models (MLLMs) deliver strong vision-language performance but at high computational cost, driven by the many visual tokens processed by the Vision Transformer (ViT) encoder. 
Existing token pruning strategies are inadequate: LLM-stage token pruning overlooks the ViT's overhead, while conventional ViT token pruning, without language guidance, risks discarding textually critical visual cues and introduces feature distortions amplified by the ViT's bidirectional attention.
To meet these challenges, we propose \textbf{IPCV}, a training-free, information-preserving compression framework for MLLM visual encoders. IPCV enables aggressive token pruning inside the ViT via \textbf{Neighbor-Guided Reconstruction (NGR)} that temporarily reconstructs pruned tokens to participate in attention with minimal overhead, then fully restores them before passing to the LLM. 
Besides, we introduce \textbf{Attention Stabilization (AS)} to further alleviate the negative influence from token pruning by approximating the K/V of pruned tokens. It can be directly applied to previous LLM-side token pruning methods to enhance their performance.
Extensive experiments show that IPCV substantially reduces end-to-end computation and outperforms state-of-the-art training-free token compression methods across diverse image and video benchmarks. 
%Our code will be released on GitHub.
Our code is provided in the supplementary material.


==> Contents/limitation.tex <==
\section{Limitations}
% As with most studies, our work is subject to certain limitations that point to directions for future research. 
Our current evaluation has primarily focused on representative MLLMs such as Qwen2-VL and InternVL3; extending validation to a wider range of architectures would provide stronger evidence of generality. 
% Moreover, although IPCV is compatible with LLM-side pruning methods, different combinations exhibit varying stability, indicating that a deeper theoretical and empirical understanding of cross-stage interactions could be beneficial.

==> Contents/theory_v1.tex <==
\section{Theoretical Analysis (Version A: Lipschitz-only)}

We analyze the perturbation introduced by IPCV's ViT-stage pruning, 
NGR-based reconstruction, and subsequent LLM-stage pruning. 
Let $\mathcal X=\{\mathbf h_{i,l_T}\}_{i=1}^L$ denote the original token set at the
final ViT block $l_T$, and let $S$ be the final token set
after NGR reconstruction and LLM-stage pruning.

% ---------------- Assumptions ----------------
\paragraph{Assumptions.}
(1) (\textbf{Downstream Lipschitz})
The MLLM mapping $F$ is $L$-Lipschitz w.r.t.~the Hausdorff distance:
\[
\|F(A)-F(B)\| \le L\, d_H(A,B), \quad \forall A,B.
\]
(2) (\textbf{Proportion pruning})
Let $\mathcal I_{\rm keep}$ be the top-$K$ indices under the 
feature-difference score
$s_i=\|\mathbf h_{i,l_p}-\mathbf h_{i,l_p-1}\|_2$,
and $\mathcal I_{\rm rem}$ be the removed indices.
Define
\[
\tau_\rho := \max_{i\in\mathcal I_{\rm rem}} s_i .
\]
(3) (\textbf{$k$-NN covering})
For each removed token $i\in\mathcal I_{\rm rem}$,
let $\mathcal N_k(i)$ be its $k$ nearest neighbors in 
$\mathcal I_{\rm keep}$ under $\ell_2$ distance at $l_p$, and define
\[
\bar\varepsilon_\rho
:= \max_{i\in \mathcal I_{\rm rem}}
\frac{1}{k}\sum_{r\in\mathcal N_k(i)}
\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2 .
\]
(4) (\textbf{Delta-smoothness})
The cross-layer increments 
$\Delta_i=\mathbf h_{i,l_T}-\mathbf h_{i,l_p}$
satisfy the Lipschitz property
\[
\|\Delta_i - \Delta_r\|_2
\le
\beta\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2 ,
\quad
\forall r\in\mathcal N_k(i).
\]
(5) (\textbf{LLM-stage pruning})
The LLM-side pruning introduces at most $\delta_{\rm llm}$ Hausdorff perturbation:
$d_H(\widehat{\mathcal X},S)\le\delta_{\rm llm}$.

% ---------------- Lemma ----------------
\begin{lemma}[NGR Pointwise Reconstruction Error]
For every removed token $i$, the NGR reconstruction
\[
\widetilde{\mathbf h}_{i,l_T}
=
\mathbf h_{i,l_p}
+
\frac{1}{k}\sum_{r\in\mathcal N_k(i)}\Delta_r
\]
satisfies
\[
\|\widetilde{\mathbf h}_{i,l_T}-\mathbf h_{i,l_T}\|_2
\;\le\;
\beta\,\bar\varepsilon_\rho .
\]
\end{lemma}

\begin{proof}[Sketch]
\[
\|\widetilde{\mathbf h}_{i,l_T}-\mathbf h_{i,l_T}\|
=
\Big\|
\frac{1}{k}\sum_{r\in\mathcal N_k(i)}(\Delta_r-\Delta_i)
\Big\|
\le
\frac{1}{k}\sum_{r\in\mathcal N_k(i)}\|\Delta_r-\Delta_i\|,
\]
then apply Assumption 4 and take the maximum over $i$.
\end{proof}

% ---------------- Theorem ----------------
\begin{theorem}[Final Output Perturbation Bound]
Let $\widehat{\mathcal X}$ be the reconstructed token set before the LLM stage.
Then
\[
\|F(\mathcal X)-F(S)\|
\;\le\;
L\big(\beta\,\bar\varepsilon_\rho + \delta_{\rm llm}\big).
\]
\end{theorem}

\begin{proof}[Sketch]
Combine the lemma with $d_H(\mathcal X,\widehat{\mathcal X})
\le\beta\bar\varepsilon_\rho$ and the LLM-stage bound 
$d_H(\widehat{\mathcal X},S)\le\delta_{\rm llm}$, then use Assumption~1.
\end{proof}


==> Contents/theory_v2.tex <==

\section{Theoretical Analysis}
%(Version B: With \texorpdfstring{$\alpha s_i$}{alpha si})
We analyze perturbations arising from IPCV, including ViT-stage pruning, NGR reconstruction, and subsequent LLM-stage pruning. 
Define 
$\mathcal{X}=\{\mathbf h_{i,l_{\text{final}}+1}\}_{i\in\mathcal{I}_{\text{keep}}}$ 
as the token set given by the output of the final ViT block $l_{\text{final}}$, where $\mathcal{I}_{\text{keep}}$ are the retained indices, 
and let $S$ denote the final token set after NGR reconstruction and LLM-side pruning.


\noindent \textbf{Assumptions.} 
We state the following assumptions to facilitate the analysis of IPCV:

\begin{enumerate}
% \item \textbf{Downstream Lipschitz.} 
% The MLLM mapping $F$ is $L$-Lipschitz w.r.t.~the Hausdorff distance:
% \[
% \|F(\mathcal X_1)-F(\mathcal X_2)\| \le L\, d_H(\mathcal X_1,\mathcal X_2), \quad \forall \mathcal X_1,\mathcal X_2.
% \]

\item \textbf{Downstream Lipschitz Continuity.} 
We assume the MLLM mapping $F$ is $L$-Lipschitz continuous with respect to the Hausdorff distance between token sets. 
Formally, for any two sets $\mathcal X_1,\mathcal X_2 \subset \mathbb{R}^d$,
\[
\|F(\mathcal X_1)-F(\mathcal X_2)\| \le L\, d_H(\mathcal X_1,\mathcal X_2),
\]
where $d_H$ denotes the Hausdorff distance induced by the Euclidean norm:
% where $d_H$ is the set distance induced by the Euclidean norm:
\(
d_H(\mathcal X_1,\mathcal X_2) := \max \\ \left\{
\begin{aligned}
&\sup_{x_1\in \mathcal X_1}\inf_{x_2\in \mathcal X_2}\|x_1-x_2\|, 
&\sup_{x_2\in \mathcal X_2}\inf_{x_1\in \mathcal X_1}\|x_1-x_2\|
\end{aligned}
\right\}.
\)


% \begin{align*}
% d_H(\mathcal X_1,\mathcal X_2) 
% &:= \max \Big\{
% \sup_{x_1\in \mathcal X_1}\inf_{x_2\in \mathcal X_2}\|x_1-x_2\|_2,\;
% \sup_{x_2\in \mathcal X_2}\inf_{x_1\in \mathcal X_1}\|x_1-x_2\|_2
% \Big\}.
% \end{align*}



\item \textbf{Proportion pruning.} 
The removed set $\mathcal I_{\rm rem}$ consists of tokens attaining the lowest $s_i$ values (see Eq.~(1)). 
Among them, the largest inter-layer variation is defined as
\[
\tau_\rho := \max_{i\in\mathcal I_{\rm rem}} s_i .
\]

\item \textbf{$k$-NN covering.} 
For each removed token $i\in\mathcal I_{\rm rem}$, let $\mathcal N_k(i)$ be its $k$ nearest neighbors in $\mathcal I_{\rm keep}$ under $\ell_2$ distance at $l_p$, and define
\[
\bar\varepsilon_\rho := \max_{i\in \mathcal I_{\rm rem}} \frac{1}{k}\sum_{r\in\mathcal N_k(i)} \|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\| .
\]

\item \textbf{Delta-smoothness with intrinsic stability.} 
The cross-layer increments 
\(
\Delta_i=\mathbf h_{i,l_{\text{final}}+1}-\mathbf h_{i,l_p}
\)
satisfy
\[
\|\Delta_i - \Delta_r\| \le \beta\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\| + \alpha\, s_i , \quad \forall r\in\mathcal N_k(i).
\]
This captures both neighbor similarity and the intrinsic small variation $s_i$ of removed tokens.

\item \textbf{LLM-stage pruning.} 
The LLM-side pruning introduces at most $\delta_{\rm llm}$ Hausdorff perturbation:
\[
d_H(\widehat{\mathcal X},S)\le\delta_{\rm llm}.
\]
\end{enumerate}

% ---------------- Lemma ----------------
\begin{lemma}[NGR Reconstruction Error with Intrinsic Term]
For every removed token $i$, the NGR reconstruction
\[
\widetilde{\mathbf h}_{i,l_{\text{final}}+1}
=
\mathbf h_{i,l_p}
+
\frac{1}{k}\sum_{r\in\mathcal N_k(i)}\Delta_r
\]
satisfies
\[
\|\widetilde{\mathbf h}_{i,l_{\text{final}}+1}-\mathbf h_{i,l_{\text{final}}+1}\|
\;\le\;
\beta\,\bar\varepsilon_\rho
+
\alpha\,\tau_\rho .
\]
\end{lemma}

\begin{proof}[Sketch]
\begin{align*}
\|\widetilde{\mathbf h}_{i,l_{\text{final}}+1}-\mathbf h_{i,l_{\text{final}}+1}\|
=
\Big\|
\frac{1}{k}\sum_{r\in\mathcal N_k(i)}(\Delta_r-\Delta_i)
\Big\| \\
\le
\frac{1}{k}\sum_{r\in\mathcal N_k(i)}\|\Delta_r-\Delta_i\|.
\end{align*}
Applying Assumption 4 yields
\[
\|\Delta_r-\Delta_i\|
\le
\beta\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|
+
\alpha s_i,
\]
and using $s_i \le \tau_\rho$ plus the definition of $\bar\varepsilon_\rho$
gives the result.
\end{proof}

% ---------------- Theorem ----------------
\begin{theorem}[Final Output Perturbation Bound]
Let $\widehat{\mathcal X}$ be the reconstructed token set before the LLM stage.
Then
\[
\|F(\mathcal X)-F(S)\|
\;\le\;
L\big(
\beta\,\bar\varepsilon_\rho
+
\alpha\,\tau_\rho
+
\delta_{\rm llm}
\big).
\]
\end{theorem}

\begin{proof}[Sketch]
The lemma implies
\[
d_H(\mathcal X,\widehat{\mathcal X})
\le\beta\bar\varepsilon_\rho+\alpha\tau_\rho.
\]
By triangle inequality,
\[
d_H(\mathcal X,S)
\le
\beta\bar\varepsilon_\rho+\alpha\tau_\rho+\delta_{\rm llm}.
\]
Applying Assumption~1 yields the final bound.
\end{proof}


==> Contents/theory_v3.tex <==
\section{Theoretical Analysis}
%(Version B: With \texorpdfstring{$\alpha s_i$}{alpha si})
We analyze perturbations arising from IPCV, including ViT-stage pruning, NGR reconstruction, and subsequent LLM-stage pruning. 
Define 
$\mathcal{X}=\{\mathbf h_{i,l_{\text{final}}+1}\}_{i\in\mathcal{I}_{\text{keep}}}$ 
as the token set given by the output of the final ViT block $l_{\text{final}}$, where $\mathcal{I}_{\text{keep}}$ are the retained indices, 
and let $S$ denote the final token set after NGR reconstruction and LLM-side pruning.


\noindent \textbf{Assumptions.} 
We state the following assumptions to facilitate the analysis of IPCV:

\begin{enumerate}
% \item \textbf{Downstream Lipschitz.} 
% The MLLM mapping $F$ is $L$-Lipschitz w.r.t.~the Hausdorff distance:
% \[
% \|F(\mathcal X_1)-F(\mathcal X_2)\| \le L\, d_H(\mathcal X_1,\mathcal X_2), \quad \forall \mathcal X_1,\mathcal X_2.
% \]

\item \textbf{Downstream Lipschitz Continuity.} 
We assume the MLLM mapping $F$ is $L$-Lipschitz continuous with respect to the Hausdorff distance between token sets. 
Formally, for any two sets $\mathcal X_1,\mathcal X_2 \subset \mathbb{R}^d$,
\[
\|F(\mathcal X_1)-F(\mathcal X_2)\| \le L\, d_H(\mathcal X_1,\mathcal X_2),
\]
where $d_H$ denotes the Hausdorff distance induced by the Euclidean norm:
% where $d_H$ is the set distance induced by the Euclidean norm:
\(
d_H(\mathcal X_1,\mathcal X_2) := \max \\ \left\{
\begin{aligned}
&\sup_{x_1\in \mathcal X_1}\inf_{x_2\in \mathcal X_2}\|x_1-x_2\|, 
&\sup_{x_2\in \mathcal X_2}\inf_{x_1\in \mathcal X_1}\|x_1-x_2\|
\end{aligned}
\right\}.
\)


% \begin{align*}
% d_H(\mathcal X_1,\mathcal X_2) 
% &:= \max \Big\{
% \sup_{x_1\in \mathcal X_1}\inf_{x_2\in \mathcal X_2}\|x_1-x_2\|_2,\;
% \sup_{x_2\in \mathcal X_2}\inf_{x_1\in \mathcal X_1}\|x_1-x_2\|_2
% \Big\}.
% \end{align*}



% \item \textbf{Proportion pruning.} 
% The removed set $\mathcal I_{\rm rem}$ consists of tokens attaining the lowest $s_i$ values (see Eq.~(1)). 
% Among them, the largest inter-layer variation is defined as
% \[
% \tau_\rho := \max_{i\in\mathcal I_{\rm rem}} s_i .
% \]

\item \textbf{$k$-NN covering.} 
For each removed token $i\in\mathcal I_{\rm rem}$, let $\mathcal N_k(i)$ be its $k$ nearest neighbors in $\mathcal I_{\rm keep}$ under $\ell_2$ distance at $l_p$, and define
\[
\bar\varepsilon_\rho := \max_{i\in \mathcal I_{\rm rem}} \frac{1}{k}\sum_{r\in\mathcal N_k(i)} \|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\| .
\]

\item \textbf{Delta-smoothness with intrinsic stability.} 
The cross-layer increments 
\(
\Delta_i=\mathbf h_{i,l_{\text{final}}+1}-\mathbf h_{i,l_p}
\)
satisfy
\[
\|\Delta_i - \Delta_r\| \le \beta\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|, \quad \forall r\in\mathcal N_k(i).
\]
This captures the neighbor similarity of removed tokens.

\item \textbf{LLM-stage pruning.} 
The LLM-side pruning introduces at most $\delta_{\rm llm}$ Hausdorff perturbation:
\[
d_H(\widehat{\mathcal X},S)\le\delta_{\rm llm}.
\]
\end{enumerate}

% ---------------- Lemma ----------------
\begin{lemma}[NGR Reconstruction Error with Intrinsic Term]
For every removed token $i$, the NGR reconstruction
\[
\widetilde{\mathbf h}_{i,l_{\text{final}}+1}
=
\mathbf h_{i,l_p}
+
\frac{1}{k}\sum_{r\in\mathcal N_k(i)}\Delta_r
\]
satisfies
\[
\|\widetilde{\mathbf h}_{i,l_{\text{final}}+1}-\mathbf h_{i,l_{\text{final}}+1}\|
\;\le\;
\beta\,\bar\varepsilon_\rho
 .
\]
\end{lemma}

\begin{proof}[Sketch]
\begin{align*}
\|\widetilde{\mathbf h}_{i,l_{\text{final}}+1}-\mathbf h_{i,l_{\text{final}}+1}\|
=
\Big\|
\frac{1}{k}\sum_{r\in\mathcal N_k(i)}(\Delta_r-\Delta_i)
\Big\| \\
\le
\frac{1}{k}\sum_{r\in\mathcal N_k(i)}\|\Delta_r-\Delta_i\|.
\end{align*}
Applying Assumption 4 yields
\[
\|\Delta_r-\Delta_i\|
\le
\beta\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|
,
\]
and the definition of $\bar\varepsilon_\rho$
gives the result.
\end{proof}

% ---------------- Theorem ----------------
\begin{theorem}[Final Output Perturbation Bound]
Let $\widehat{\mathcal X}$ be the reconstructed token set before the LLM stage.
Then
\[
\|F(\mathcal X)-F(S)\|
\;\le\;
L\big(
\beta\,\bar\varepsilon_\rho
+
\delta_{\rm llm}
\big).
\]
\end{theorem}

\begin{proof}[Sketch]
The lemma implies
\[
d_H(\mathcal X,\widehat{\mathcal X})
\le\beta\bar\varepsilon_\rho.
\]
By triangle inequality,
\[
d_H(\mathcal X,S)
\le
\beta\bar\varepsilon_\rho+\delta_{\rm llm}.
\]
Applying Assumption~1 yields the final bound.
\end{proof}







\begin{lemma}[Delta-smoothness]
Let \(G\) denote the mapping that carries the set of token embeddings at layer \(l_p\)
to the set of token embeddings at layer \(l_{\text{final}}+1\) (the ViT tail).
Assume \(G\) is Hausdorff-Lipschitz with constant \(K_{\mathrm{ViT}}\ge0\), i.e.
for any two token sets \(X,Y\) at layer \(l_p\),
\[
d_H\big(G(X),G(Y)\big)\le K_{\mathrm{ViT}}\,d_H(X,Y).
\]
Let
\(\Delta_i=\mathbf h_{i,l_{\text{final}}+1}-\mathbf h_{i,l_p}\)
and \(\Delta_r=\mathbf h_{r,l_{\text{final}}+1}-\mathbf h_{r,l_p}\).
Then for any two token positions \(i,r\) at layer \(l_p\) it holds that
\[
\|\Delta_i-\Delta_r\|_2 \le (K_{\mathrm{ViT}}+1)\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2.
\]
In particular one may take \(\beta=K_{\mathrm{ViT}}+1\) in the bound
\(\|\Delta_i-\Delta_r\|_2\le\beta\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2\).
\end{lemma}

\begin{proof}
Let \(X\) be the full token set at layer \(l_p\), and let \(X^{(i\to r)}\) be the
set obtained from \(X\) by replacing the token at position \(i\) with \(\mathbf h_{r,l_p}\)
(keeping all other tokens identical). By definition of the Hausdorff distance,
\[
d_H(X,\,X^{(i\to r)}) \le \|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2.
\]
Applying the Hausdorff-Lipschitz property of \(G\) yields
\[
d_H\big(G(X),\,G(X^{(i\to r)})\big) \le K_{\mathrm{ViT}}\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2.
\]
Under the positional correspondence between layers, the outputs at the positions
corresponding to \(i\) and \(r\) satisfy the pointwise bound
\[
\big\|\mathbf h_{i,l_{\text{final}}+1}-\mathbf h_{r,l_{\text{final}}+1}\big\|_2
\le K_{\mathrm{ViT}}\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2.
\]
Now write
\[
\Delta_i-\Delta_r
= (\mathbf h_{i,l_{\text{final}}+1}-\mathbf h_{r,l_{\text{final}}+1})
  -(\mathbf h_{i,l_p}-\mathbf h_{r,l_p}).
\]
Taking norms and using the triangle inequality gives
\[
\|\Delta_i-\Delta_r\|_2
\le \big\|\mathbf h_{i,l_{\text{final}}+1}-\mathbf h_{r,l_{\text{final}}+1}\big\|_2
    +\big\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\big\|_2
\le (K_{\mathrm{ViT}}+1)\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2,
\]
which proves the lemma.
\end{proof}


==> Contents/theory_v4.tex <==

\section{Theoretical Analysis}
%(Version B: With \texorpdfstring{$\alpha s_i$}{alpha si})
We analyze perturbations arising from IPCV, including ViT-stage pruning, NGR reconstruction, and subsequent LLM-stage pruning. 
Define 
$\mathcal{X}=\{\mathbf h_{i,l_{\text{final}}+1}\}_{i\in\mathcal{I}_{\text{keep}}}$ 
as the token set given by the output of the final ViT block $l_{\text{final}}$, where $\mathcal{I}_{\text{keep}}$ are the retained indices, 
and let $S$ denote the final token set after NGR reconstruction and LLM-side pruning.


\noindent \textbf{Assumptions.} 
We state the following assumptions to facilitate the analysis of IPCV:

\begin{enumerate}
% \item \textbf{Downstream Lipschitz.} 
% The MLLM mapping $F$ is $L$-Lipschitz w.r.t.~the Hausdorff distance:
% \[
% \|F(\mathcal X_1)-F(\mathcal X_2)\| \le L\, d_H(\mathcal X_1,\mathcal X_2), \quad \forall \mathcal X_1,\mathcal X_2.
% \]

\item \textbf{Downstream Lipschitz Continuity.} 
We assume the ViT mapping $F$ is $L$-Lipschitz continuous with respect to the Hausdorff distance between token sets. 
Formally, for any two sets $\mathcal X_1,\mathcal X_2 \subset \mathbb{R}^d$,
\[
\|F(\mathcal X_1)-F(\mathcal X_2)\| \le L\, d_H(\mathcal X_1,\mathcal X_2),
\]
where $d_H$ denotes the Hausdorff distance induced by the Euclidean norm:
% where $d_H$ is the set distance induced by the Euclidean norm:
\(
d_H(\mathcal X_1,\mathcal X_2) := \max \\ \left\{
\begin{aligned}
&\sup_{x_1\in \mathcal X_1}\inf_{x_2\in \mathcal X_2}\|x_1-x_2\|, 
&\sup_{x_2\in \mathcal X_2}\inf_{x_1\in \mathcal X_1}\|x_1-x_2\|
\end{aligned}
\right\}.
\)




% \begin{align*}
% d_H(\mathcal X_1,\mathcal X_2) 
% &:= \max \Big\{
% \sup_{x_1\in \mathcal X_1}\inf_{x_2\in \mathcal X_2}\|x_1-x_2\|_2,\;
% \sup_{x_2\in \mathcal X_2}\inf_{x_1\in \mathcal X_1}\|x_1-x_2\|_2
% \Big\}.
% \end{align*}



% \item \textbf{Proportion pruning.} 
% The removed set $\mathcal I_{\rm rem}$ consists of tokens attaining the lowest $s_i$ values (see Eq.~(1)). 
% Among them, the largest inter-layer variation is defined as
% \[
% \tau_\rho := \max_{i\in\mathcal I_{\rm rem}} s_i .
% \]




\item \textbf{Bounded embeddings.} There exists $B>0$ s.t.\ all token embeddings satisfy $\|x\|_2\le B$.



% \item \textbf{$k$-NN covering.} 
% For each removed token $i\in\mathcal I_{\rm rem}$, let $\mathcal N_k(i)$ be its $k$ nearest neighbors in $\mathcal I_{\rm keep}$ under $\ell_2$ distance at $l_p$, and define
% \[
% \bar\varepsilon_\rho := \max_{i\in \mathcal I_{\rm rem}} \frac{1}{k}\sum_{r\in\mathcal N_k(i)} \|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\| .
% \]

% \item \textbf{Delta-smoothness with intrinsic stability.} 
% The cross-layer increments 
% \(
% \Delta_i=\mathbf h_{i,l_{\text{final}}+1}-\mathbf h_{i,l_p}
% \)
% satisfy
% \[
% \|\Delta_i - \Delta_r\| \le \beta\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|, \quad \forall r\in\mathcal N_k(i).
% \]
% This captures the neighbor similarity of removed tokens.

% \item \textbf{LLM-stage pruning.} 
% The LLM-side pruning introduces at most $\delta_{\rm llm}$ Hausdorff perturbation:
% \[
% d_H(\widehat{\mathcal X},S)\le\delta_{\rm llm}.
% \]
\end{enumerate}

% ---------------- Lemma ----------------

\begin{lemma}[Delta-smoothness]
Let \(G\) denote the mapping that carries the set of token embeddings at layer \(l_p\)
to the set of token embeddings at layer \(l_{\text{final}}+1\) (the ViT tail).
Assume \(G\) is Hausdorff-Lipschitz with constant \(K_{\mathrm{ViT}}\ge0\), i.e.
for any two token sets \(X,Y\) at layer \(l_p\),
\[
d_H\big(G(X),G(Y)\big)\le K_{\mathrm{ViT}}\,d_H(X,Y).
\]
Let
\(\Delta_i=\mathbf h_{i,l_{\text{final}}+1}-\mathbf h_{i,l_p}\)
and \(\Delta_r=\mathbf h_{r,l_{\text{final}}+1}-\mathbf h_{r,l_p}\).
Then for any two token positions \(i,r\) at layer \(l_p\) it holds that
\[
\|\Delta_i-\Delta_r\|_2 \le (K_{\mathrm{ViT}}+1)\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2.
\]
In particular one may take \(\beta=K_{\mathrm{ViT}}+1\) in the bound
\(\|\Delta_i-\Delta_r\|_2\le\beta\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2\).
\end{lemma}

\begin{proof}
Let \(X\) be the full token set at layer \(l_p\), and let \(X^{(i\to r)}\) be the
set obtained from \(X\) by replacing the token at position \(i\) with \(\mathbf h_{r,l_p}\)
(keeping all other tokens identical). By definition of the Hausdorff distance,
\[
d_H(X,\,X^{(i\to r)}) \le \|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2.
\]
Applying the Hausdorff-Lipschitz property of \(G\) yields
\[
d_H\big(G(X),\,G(X^{(i\to r)})\big) \le K_{\mathrm{ViT}}\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2.
\]
Under the positional correspondence between layers, the outputs at the positions
corresponding to \(i\) and \(r\) satisfy the pointwise bound
\[
\big\|\mathbf h_{i,l_{\text{final}}+1}-\mathbf h_{r,l_{\text{final}}+1}\big\|_2
\le K_{\mathrm{ViT}}\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2.
\]
Now write
\[
\Delta_i-\Delta_r
= (\mathbf h_{i,l_{\text{final}}+1}-\mathbf h_{r,l_{\text{final}}+1})
  -(\mathbf h_{i,l_p}-\mathbf h_{r,l_p}).
\]
Taking norms and using the triangle inequality gives
\[
\|\Delta_i-\Delta_r\|_2
\le \big\|\mathbf h_{i,l_{\text{final}}+1}-\mathbf h_{r,l_{\text{final}}+1}\big\|_2
    +\big\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\big\|_2
\le (K_{\mathrm{ViT}}+1)\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2,
\]
which proves the lemma.
\end{proof}


\begin{remark}
Combining the lemma with the bounded-embedding assumption ($\|x\|_2\le B$) yields
$\|\Delta_i-\Delta_r\|_2 \le \beta\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2
\le 2\beta B$.
\end{remark}

% \begin{remark}
% Combining the lemma with the bounded-embedding assumption ($\|x\|_2\le B$) yields
% $\|\Delta_i-\Delta_r\|_2 \le (K_{\mathrm{ViT}}+1)\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2
% \le 2B(K_{\mathrm{ViT}}+1)$.
% \end{remark}








% \begin{lemma}[NGR Reconstruction Error with Intrinsic Term]
% For every removed token $i$, the NGR reconstruction
% \[
% \widetilde{\mathbf h}_{i,l_{\text{final}}+1}
% =
% \mathbf h_{i,l_p}
% +
% \frac{1}{k}\sum_{r\in\mathcal N_k(i)}\Delta_r
% \]
% satisfies
% \[
% \|\widetilde{\mathbf h}_{i,l_{\text{final}}+1}-\mathbf h_{i,l_{\text{final}}+1}\|
% \;\le\;
% \beta\,\bar\varepsilon_\rho
% \;\le\; 2B\beta,
% \]
% where $B>0$ is the embedding bound from Assumption (Bounded embeddings).
% \end{lemma}

% \begin{proof}[Sketch]
% \begin{align*}
% \|\widetilde{\mathbf h}_{i,l_{\text{final}}+1}-\mathbf h_{i,l_{\text{final}}+1}\|
% &=
% \Big\|
% \frac{1}{k}\sum_{r\in\mathcal N_k(i)}(\Delta_r-\Delta_i)
% \Big\| \\
% &\le
% \frac{1}{k}\sum_{r\in\mathcal N_k(i)}\|\Delta_r-\Delta_i\|.
% \end{align*}
% Applying Assumption 4 yields
% \[
% \|\Delta_r-\Delta_i\|
% \le
% \beta\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|.
% \]
% Taking the average and the maximum over $i$ gives the first inequality:
% \[
% \|\widetilde{\mathbf h}_{i,l_{\text{final}}+1}-\mathbf h_{i,l_{\text{final}}+1}\|
% \le\beta\,\bar\varepsilon_\rho.
% \]
% Under the bounded-embedding assumption $\|\mathbf h\|_2\le B$ for all tokens,
% we have $\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|\le 2B$, hence
% $\bar\varepsilon_\rho\le 2B$, and therefore
% \[
% \|\widetilde{\mathbf h}_{i,l_{\text{final}}+1}-\mathbf h_{i,l_{\text{final}}+1}\|
% \le \beta\,\bar\varepsilon_\rho \le 2B\beta,
% \]
% as claimed.
% \end{proof}



\begin{lemma}[NGR Reconstruction Error]
Under the bounded-embedding assumption \(\|x\|_2 \le B\) and the \(\Delta\)-smoothness bound
\(\|\Delta_i - \Delta_r\|_2 \le \beta\,\|\mathbf h_{i,l_p} - \mathbf h_{r,l_p}\|_2\),
the NGR reconstruction satisfies, for each removed token \(i\),
\[
\|\widetilde{\mathbf h}_{i,l_{\text{final}}+1} - \mathbf h_{i,l_{\text{final}}+1}\|_2
\;\le\; 2B\beta.
\]
Consequently the Hausdorff distance between the original final-layer set $\mathcal X$ and
the reconstructed set $\widehat{\mathcal X}$ obeys
\[
d_H(\mathcal X,\widehat{\mathcal X}) \le 2B\beta.
\]
\end{lemma}

\begin{proof}[Sketch]
\[
\widetilde{\mathbf h}_{i,l_{\text{final}}+1}
- \mathbf h_{i,l_{\text{final}}+1}
= \frac{1}{k}\sum_{r\in\mathcal N_k(i)}(\Delta_r - \Delta_i),
\]
so by triangle inequality and smoothness,
\[
\|\widetilde{\mathbf h}_{i,l_{\text{final}}+1} - \mathbf h_{i,l_{\text{final}}+1}\|
\le \frac{1}{k} \sum_{r\in\mathcal N_k(i)} \|\Delta_r - \Delta_i\|
\le \frac{1}{k} \sum_{r\in\mathcal N_k(i)} \beta\,\|\mathbf h_{i,l_p} - \mathbf h_{r,l_p}\|.
\]
Since \(\|\mathbf h_{i,l_p} - \mathbf h_{r,l_p}\| \le \|\mathbf h_{i,l_p}\| + \|\mathbf h_{r,l_p}\| \le 2B\),
each term in the sum is at most \(2B\beta\), and averaging gives the bound \(2B\beta\).
\end{proof}


\paragraph{Discussion.}
This bound isolates the ViT-stage error introduced by IPCV (pruning + NGR). The bound is
conservative (worst-case); in practice one can measure the dataset-dependent average neighbor
distance to obtain a much tighter empirical bound (see supp.).












==> Contents/theory_v5.tex <==

\section{Theoretical Analysis}
This section provides a theoretical analysis of perturbations arising from ViT-stage pruning and Reintegration.

% We analyze perturbations arising from IPCV, including ViT-stage pruning and NGR reconstruction. 

% \noindent \textbf{Assumptions.} 
% To facilitate the theoretical analysis, the following assumptions are introduced:
% We state the following assumptions to facilitate the analysis:




% \item \textbf{Downstream Lipschitz Continuity.} 
% We assume the ViT model mapping $F$ is $L_{\mathrm{ViT}}$-Lipschitz continuous with respect to the Hausdorff distance between token sets. 
% Formally, for any two sets $\mathcal X_1,\mathcal X_2 \subset \mathbb{R}^d$,
% \[
% \|F(\mathcal X_1)-F(\mathcal X_2)\| \le L_{\mathrm{ViT}}\, d_H(\mathcal X_1,\mathcal X_2),
% \]
% where $d_H$ denotes the Hausdorff distance induced by the Euclidean norm:
% % where $d_H$ is the set distance induced by the Euclidean norm:
% \(
% d_H(\mathcal X_1,\mathcal X_2) := \max \\ \left\{
% \begin{aligned}
% &\sup_{x_1\in \mathcal X_1}\inf_{x_2\in \mathcal X_2}\|x_1-x_2\|, 
% &\sup_{x_2\in \mathcal X_2}\inf_{x_1\in \mathcal X_1}\|x_1-x_2\|
% \end{aligned}
% \right\}.
% \)



\begin{assumption}[Hausdorff-Lipschitz Continuity]\label{assump:hausdorff}
We assume the ViT mapping $F$ from layer $l_p$ to $l_{\text{final}}+1$ is $L_{\mathrm{ViT}}$-Lipschitz with respect to the Hausdorff distance.
Formally, for any two sets $\mathcal X_1, \mathcal X_2 \subset \mathbb{R}^d$,
\[
d_H(F(\mathcal X_1), F(\mathcal X_2)) \le L_{\mathrm{ViT}}\, d_H(\mathcal X_1,\mathcal X_2),
\]
where $d_H$ denotes the Hausdorff distance under the Euclidean norm:
% where $d_H$ is the set distance induced by the Euclidean norm:
\(
d_H(\mathcal X_1,\mathcal X_2) := \max \\ \left\{
\begin{aligned}
&\sup_{x_1\in \mathcal X_1}\inf_{x_2\in \mathcal X_2}\|x_1-x_2\|_2, 
&\sup_{x_2\in \mathcal X_2}\inf_{x_1\in \mathcal X_1}\|x_1-x_2\|_2
\end{aligned}
\right\}.
\)

\end{assumption}




\begin{assumption}[Bounded embeddings]\label{assump:bounded}
There exists a constant $B>0$ s.t.\ all token embeddings satisfy $\|x\|_2\le B$.
\end{assumption}




% ---------------- Lemma ----------------

% \begin{lemma}[Delta-smoothness]
% %(Assumption: $F$ is $L_{\mathrm{ViT}}$-Hausdorff-Lipschitz from layer $l_p$ to $l_{\mathrm{final}}+1$)
% % Under the Hausdorff-Lipschitz Continuity assumption, define
% % Under the ViT Lipschitz assumption, from pruning layer $l_p$ to final model output $l_{\mathrm{final}}+1$,
% % denote
% For any two token positions $i,r$, we define
% \[
% \Delta_i=\mathbf h_{i,l_{\mathrm{final}}+1}-\mathbf h_{i,l_p},\qquad
% \Delta_r=\mathbf h_{r,l_{\mathrm{final}}+1}-\mathbf h_{r,l_p}.
% \]
% Then, under Assumption~\ref{assump:hausdorff}, the following bound holds:
% \[
% \|\Delta_i-\Delta_r\|_2 \le (L_{\mathrm{ViT}}+1)\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2.
% \]
% \end{lemma}

% \begin{proof}
% % Let $X$ be the full token set at layer $l_p$ and let $X^{(i\to r)}$ be $X$ with the $i$-th token
% % replaced by $\mathbf h_{r,l_p}$. By definition,
% Consider the full token set $X$ at layer $l_p$, and define $X^{(i\to r)}$ as the set where the $i$-th token is replaced by $\mathbf h_{r,l_p}$. By the above construction,
% \[
% d_H(X,X^{(i\to r)}) \le \|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2.
% \]
% From Assumption~\ref{assump:hausdorff}, it follows that
% \[
% d_H\big(F(X),F(X^{(i\to r)})\big) \le L_{\mathrm{ViT}}\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2.
% \]
% By positional correspondence the outputs at the positions corresponding to $i$ and $r$ satisfy
% \(
% \|\mathbf h_{i,l_{\mathrm{final}}+1}-\mathbf h_{r,l_{\mathrm{final}}+1}\|_2
% \le L_{\mathrm{ViT}}\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2.
% \)
% Therefore
% \[
% \begin{aligned}
% \|\Delta_i-\Delta_r\|_2
% &= \|(\mathbf h_{i,l_{\mathrm{final}}+1}-\mathbf h_{r,l_{\mathrm{final}}+1})
%      -(\mathbf h_{i,l_p}-\mathbf h_{r,l_p})\|_2 \\
% &\le \|\mathbf h_{i,l_{\mathrm{final}}+1}-\mathbf h_{r,l_{\mathrm{final}}+1}\|_2
%      +\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2 \\
% &\le (L_{\mathrm{ViT}}+1)\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2,
% \end{aligned}
% \]
% which proves the claim.
% \end{proof}

% \begin{remark}
% Setting $\beta := L_{\mathrm{ViT}}+1$ yields the commonly-used form
% \(\|\Delta_i-\Delta_r\|_2\le\beta\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2\).
% Combining this with the bounded-embedding assumption $\|x\|_2\le B$ gives the absolute bound
% \(\|\Delta_i-\Delta_r\|_2 \le 2B\beta\).
% \end{remark}




\begin{lemma}[Pointwise deviation bound under pruning]
% Let $X$ be the full token set at layer $l_p$ and $Y\subset X$ the kept set after pruning.
% For any $i\in X$ and any $r\in Y$ define
Consider the full token set $X$ at layer $l_p$, with $Y\subset X$ denoting the subset retained after pruning.
For any $i\in X$ and $r\in Y$, we define the token update by:
\[
\Delta_i := F_i(X)-\mathbf h_{i,l_p},\qquad
\Delta_r := F_r(Y)-\mathbf h_{r,l_p},
\]
% where $F_j(\cdot)$ denotes the final-layer output at position $j$ given the input set.
% Under Assumption~\ref{assump:hausdorff} and Assumption~\ref{assump:bounded} we have
where $F_j(\cdot)$ denotes the final-layer output at position $j$ given the input set.
Then the following bound holds:
\[
\|\Delta_i-\Delta_r\|_2
\le
\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2
+ L_{\mathrm{ViT}}\,d_H(X,Y) + 2B.
\]
\end{lemma}

\begin{proof}
% By Assumption~\ref{assump:hausdorff}, $d_H(F(X),F(Y))\le L_{\mathrm{ViT}}\,d_H(X,Y)$.
% Hence for the output $F_i(X)\in F(X)$ and any chosen $r\in Y$ we have
By Assumption~\ref{assump:hausdorff}, $d_H(F(X),F(Y))\le L_{\mathrm{ViT}}\,d_H(X,Y)$.
Consequently, for any output token $F_i(X)\in F(X)$ and any $r\in Y$, we have
\[
\|F_i(X)-F_r(Y)\|_2 \le L_{\mathrm{ViT}}\,d_H(X,Y) + \mathrm{diam}\big(F(Y)\big).
\]
Under Assumption~\ref{assump:bounded} the diameter of $F(Y)$ satisfies $\mathrm{diam}(F(Y))\le 2B$, hence
\[
\|F_i(X)-F_r(Y)\|_2 \le L_{\mathrm{ViT}}\,d_H(X,Y) + 2B.
\]
Therefore, the deviation of token update is bounded by
\[
\begin{aligned}
\|\Delta_i-\Delta_r\|_2
&= \|F_i(X)-F_r(Y) -(\mathbf h_{i,l_p}-\mathbf h_{r,l_p})\|_2 \\
&\le \|F_i(X)-F_r(Y)\|_2 + \|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2 \\
&\le \|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2 + L_{\mathrm{ViT}}\,d_H(X,Y) + 2B,
\end{aligned}
\]
as claimed.
\end{proof}





\begin{remark} \label{remark:pointwise-bound}
% Using the bounded-embedding Assumption~\ref{assump:bounded}, the pointwise bound
% \[
% \|\Delta_i-\Delta_r\|_2
% \le
% \|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2
% + L_{\mathrm{ViT}}\,d_H(X,Y) + 2B
% \]
% implies the worst-case constant bound
% \[
% \|\Delta_i-\Delta_r\|_2 \le 2B\,(L_{\mathrm{ViT}}+2).
% \]
% Since $\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2\le 2B$ and $d_H(X,Y)\le 2B$.

By Assumption~\ref{assump:bounded}, both $\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|_2$ and $d_H(X,Y)$ are at most $2B$. 
Substituting these bounds into the pointwise inequality gives
\[
\|\Delta_i-\Delta_r\|_2 \le 2B\,(L_{\mathrm{ViT}}+2).
\]



\end{remark}









% \begin{lemma}[NGR Reconstruction Error with Intrinsic Term]
% For every removed token $i$, the NGR reconstruction
% \[
% \widetilde{\mathbf h}_{i,l_{\text{final}}+1}
% =
% \mathbf h_{i,l_p}
% +
% \frac{1}{k}\sum_{r\in\mathcal N_k(i)}\Delta_r
% \]
% satisfies
% \[
% \|\widetilde{\mathbf h}_{i,l_{\text{final}}+1}-\mathbf h_{i,l_{\text{final}}+1}\|
% \;\le\;
% \beta\,\bar\varepsilon_\rho
% \;\le\; 2B\beta,
% \]
% where $B>0$ is the embedding bound from Assumption (Bounded embeddings).
% \end{lemma}

% \begin{proof}[Sketch]
% \begin{align*}
% \|\widetilde{\mathbf h}_{i,l_{\text{final}}+1}-\mathbf h_{i,l_{\text{final}}+1}\|
% &=
% \Big\|
% \frac{1}{k}\sum_{r\in\mathcal N_k(i)}(\Delta_r-\Delta_i)
% \Big\| \\
% &\le
% \frac{1}{k}\sum_{r\in\mathcal N_k(i)}\|\Delta_r-\Delta_i\|.
% \end{align*}
% Applying Assumption 4 yields
% \[
% \|\Delta_r-\Delta_i\|
% \le
% \beta\,\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|.
% \]
% Taking the average and the maximum over $i$ gives the first inequality:
% \[
% \|\widetilde{\mathbf h}_{i,l_{\text{final}}+1}-\mathbf h_{i,l_{\text{final}}+1}\|
% \le\beta\,\bar\varepsilon_\rho.
% \]
% Under the bounded-embedding assumption $\|\mathbf h\|_2\le B$ for all tokens,
% we have $\|\mathbf h_{i,l_p}-\mathbf h_{r,l_p}\|\le 2B$, hence
% $\bar\varepsilon_\rho\le 2B$, and therefore
% \[
% \|\widetilde{\mathbf h}_{i,l_{\text{final}}+1}-\mathbf h_{i,l_{\text{final}}+1}\|
% \le \beta\,\bar\varepsilon_\rho \le 2B\beta,
% \]
% as claimed.
% \end{proof}


\begin{theorem}[NGR Reconstruction Error]
% The NGR reconstruction satisfies, for each removed token \(i\),
%admits the bound
For each removed token \(i\), the NGR reconstruction satisfies the bound
\[
\|\widetilde{\mathbf h}_{i,l_{\text{final}}+1} - \mathbf h_{i,l_{\text{final}}+1}\|_2
\;\le\; 2B\,(L_{\mathrm{ViT}}+2).
\]
Here $\widetilde{\mathbf h}_{i,l_{\text{final}}+1}$ denotes the reconstructed hidden state
of pruned token $i$ via NGR, and $\mathbf h_{i,l_{\text{final}}+1}$ the true hidden state without pruning.
Consequently, the Hausdorff distance between the original final-layer set $\mathcal X$ and
the reconstructed set $\widehat{\mathcal X}$ is bounded by
\[
d_H(\mathcal X,\widehat{\mathcal X}) \le 2B\,(L_{\mathrm{ViT}}+2).
\]
\end{theorem}

\begin{proof}[Sketch]
Recall that
\[
\widetilde{\mathbf h}_{i,l_{\text{final}}+1}
- \mathbf h_{i,l_{\text{final}}+1}
= \frac{1}{k}\sum_{r\in\mathcal N_k(i)}(\Delta_r - \Delta_i),
\]
By the triangle inequality,
\[
\|\widetilde{\mathbf h}_{i,l_{\text{final}}+1} - \mathbf h_{i,l_{\text{final}}+1}\|_2
\le \frac{1}{k} \sum_{r\in\mathcal N_k(i)} \|\Delta_r - \Delta_i\|_2.
\]
From the Remark~\ref{remark:pointwise-bound} we have the worst-case bound
\(\|\Delta_r-\Delta_i\|_2 \le 2B\,(L_{\mathrm{ViT}}+2)\) for any \(r\). Thus each term
in the sum is  bounded by \(2B(L_{\mathrm{ViT}}+2)\), and averaging yields the stated bound.
\end{proof}




% \begin{lemma}[NGR Reconstruction Error]
% Under the bounded-embedding assumption \(\|x\|_2 \le B\) and the \(\Delta\)-smoothness bound
% \(\|\Delta_i - \Delta_r\|_2 \le \beta\,\|\mathbf h_{i,l_p} - \mathbf h_{r,l_p}\|_2\),
% the NGR reconstruction satisfies, for each removed token \(i\),
% \[
% \|\widetilde{\mathbf h}_{i,l_{\text{final}}+1} - \mathbf h_{i,l_{\text{final}}+1}\|_2
% \;\le\; 2B\beta.
% \]
% where $\widetilde{\mathbf h}_{i,l_{\text{final}}+1}$ denotes the reconstructed hidden state of pruned token $i$ via NGR, 
% and $\mathbf h_{i,l_{\text{final}}+1}$ the true hidden state without pruning.
% Consequently the Hausdorff distance between the original final-layer set $\mathcal X$ and
% the reconstructed set $\widehat{\mathcal X}$ obeys
% \[
% d_H(\mathcal X,\widehat{\mathcal X}) \le 2B\beta.
% \]
% \end{lemma}

% \begin{proof}[Sketch]
% \[
% \widetilde{\mathbf h}_{i,l_{\text{final}}+1}
% - \mathbf h_{i,l_{\text{final}}+1}
% = \frac{1}{k}\sum_{r\in\mathcal N_k(i)}(\Delta_r - \Delta_i),
% \]
% so by triangle inequality and smoothness,

% \begin{align*}
% \|\widetilde{\mathbf h}_{i,l_{\text{final}}+1} - \mathbf h_{i,l_{\text{final}}+1}\|_2
% \le \frac{1}{k} \sum_{r\in\mathcal N_k(i)} \|\Delta_r - \Delta_i\|_2   \\
% \le \frac{1}{k} \sum_{r\in\mathcal N_k(i)} \beta\,\|\mathbf h_{i,l_p} - \mathbf h_{r,l_p}\|_2.
% \end{align*}

% Since \(\|\mathbf h_{i,l_p} - \mathbf h_{r,l_p}\| \le \|\mathbf h_{i,l_p}\| + \|\mathbf h_{r,l_p}\| \le 2B\),
% each term in the sum is at most \(2B\beta\), and averaging gives the bound \(2B\beta\).
% \end{proof}


% \paragraph{Discussion.}
% This bound isolates the ViT-stage error introduced by IPCV (pruning + NGR). The bound is
% conservative (worst-case); in practice one can measure the dataset-dependent average neighbor
% distance to obtain a much tighter empirical bound (see supp.).












==> author-kit-CVPR2026-v1-latex-/preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> author-kit-CVPR2026-v1-latex-/sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> author-kit-CVPR2026-v1-latex-/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets the figure captions and references in a smaller font.
The reason why such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The review process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in 11 pages.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler that should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use the options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Use fractional references (\eg, this line is $087.5$), although in most cases the approximate location would be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please, number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for the reader to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean that some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not mean that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of our previous paper [1], and show that it is inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of the paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time that covers similar or overlapping material, you may need to refer to that submission to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, do not assume that the reviewers will read this material.

Sometimes your paper is about a problem that you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think that it is likely that the new article was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
However, for your results, you should not identify yourself and should not mention your participation in the challenge.
Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison with other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has only two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> author-kit-CVPR2026-v1-latex-/sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> author-kit-CVPR2026-v1-latex-/sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
